Searching Similarity Measure for Binarized Neural Networks

Being a promising model to be deployed in resource-limited devices, Binarized Neural Networks (BNNs) have drawn extensive attention from both academic and industry. However, comparing to the full-precision deep neural networks (DNNs), BNNs suffer from non-trivial accuracy degradation, limiting its applicability in various domains. This is partially because existing network components, such as the similarity measure, are specially designed for DNNs, and might be sub-optimal for BNNs. In this work, we focus on the key component of BNNs -- the similarity measure, which quantifies the distance between input feature maps and filters, and propose an automatic searching method, based on genetic algorithm, for BNN-tailored similarity measure. Evaluation results on Cifar10 and Cifar100 using ResNet, NIN and VGG show that most of the identified similarty measure can achieve considerable accuracy improvement (up to 3.39%) over the commonly-used cross-correlation approach.

==> ak.tex <==
 is extremely effective and thus is the standard in state of the art template matching algorithms
 
 There are surveys collected binary similarity and dissimilarity measures used over the last century and reveal their correlations\cite{}. 
 GA is an appealing approach to obtain high-quality solutions for an optimization problem thanks to its ability to deliver a good solution fast-enough.


GA can explore the search space in many directions simultaneously which is ideal to parallelize the algorithms for implementation.

The GA technique outperforms other traditional methods in most problems, as it is a more general and a flexible method with the capability of searching over a wide solution space and at the same time avoiding falling into a local minimum. Thus, it has the potential for finding an optimal or a near-optimal combination of the parameter values. This algorithm can perform a random search within a predefined search space and can solve a specific problem as well.


Since then, many variants of genetic algorithms have been developed and applied to a wide range of optimization problems, from graph coloring to pattern recognition, from discrete systems (such as the travelling salesman problem) to continuous systems (e.g., the efficient design of airfoil in aerospace engineering), and from financial markets to multi-objective engineering optimization.

There are many advantages of genetic algorithms over traditional optimization algorithms. Two most notable are: the ability of dealing with complex problems and parallelism. Genetic algorithms can deal with various types of optimization, whether the objective (fitness) function is stationary or non-stationary (change with time), linear or nonlinear, continuous or discontinuous, or with random noise. Because multiple offsprings in a population act like independent agents, the population (or any subgroup) can explore the search space in many directions simultaneously. This feature makes it ideal to parallelize the algorithms for implementation. Different parameters and even different groups of encoded strings can be manipulated at the same time.
